Motion of small bodies in general relativity: foundations and implementations of the self-force

Extreme mass-ratio inspirals, in which solar-mass compact bodies spiral into supermassive black holes, are an important potential source for gravitational wave detectors. Because of the extreme mass-ratio, one can model these systems using perturbation theory. However, in order to relate the motion of the small body to the emitted waveform, one requires a model that is accurate on extremely long timescales. Additionally, in order to avoid intractable divergences, one requires a model that treats the small body as asymptotically small rather than exactly pointlike. Both of these difficulties can be resolved by using techniques of singular perturbation theory. I begin this dissertation with an analysis of singular perturbation theory on manifolds, including the common techniques of matched asymptotic expansions and two-timescale expansions. I then formulate a systematic asymptotic expansion in which the metric perturbation due to the body is expanded while a representative worldline is held fixed, and I contrast it with a regular expansion in which both the metric and the worldline must be expanded. This results in an approximation that is potentially uniformly accurate on long timescales. The equation of motion for the body's fixed worldline is determined by performing a local-in-space expansion in the neighbourhood of the body. Using this local expansion as boundary data, I construct a global solution to the perturbative Einstein equation. To concretely characterize orbits, I next devise a relativistic generalization of the Newtonian method of osculating orbits. Making use of this method and two-timescale expansions, I examine the utility of adiabatic approximations that can forgo an explicit calculation of the force.

==> buffer_expansions.tex <==
\chapter{Expansions of the Riemann tensor and related quantities}\label{general_expansions}
\section{General expansions in powers of the metric perturbation}
The part of the Ricci tensor that is quadratic in the perturbation $h$ is written as
\begin{align}
\delta^2R_{\alpha\beta}[h] &=-\tfrac{1}{2}\bar h^{\mu\nu}{}_{;\nu}\left(2h_{\mu(\alpha;\beta)}-h_{\alpha\beta;\mu}\right) +\tfrac{1}{4}h^{\mu\nu}{}_{;\alpha}h_{\mu\nu;\beta}+\tfrac{1}{2}h^{\mu}{}_{\beta}{}^{;\nu}\left(h_{\mu\alpha;\nu} -h_{\nu\alpha;\mu}\right)\nonumber\\
&\quad-\tfrac{1}{2}h^{\mu\nu}\left(2h_{\mu(\alpha;\beta)\nu}-h_{\alpha\beta;\mu\nu}-h_{\mu\nu;\alpha\beta}\right).
\end{align}

\section{Expansions necessary for the second-order wave equation in the buffer region}\label{second-order expansions}
I present here various expansions used in solving the second-order Einstein equation in Sec.~\ref{buffer_expansion2}.

I require an expansion of $\delta^2 R\coeff{0}_{\alpha\beta}[\hmn{}{1}]$ in powers of the Fermi radial coordinate $r$, where for a function $f$, $\delta^2 R\coeff{0}_{\alpha\beta}[f]$ consists of $\delta^2 R_{\alpha\beta}[f]$ with the acceleration $a^\mu$ set to zero. Explicitly, I require the coefficients in the expansion
\begin{align}
\delta^2R\coeff{0}_{\alpha\beta}[\hmn{}{1}] &= \frac{1}{r^4}\ddR{\alpha\beta}{0,-4}{\hmn{}{1}}\!\! +\frac{1}{r^3}\ddR{\alpha\beta}{0,-3}{\hmn{}{1}}\ \ \nonumber\\
&\quad+\frac{1}{r^2}\ddR{\alpha\beta}{0,-2}{\hmn{}{1}} +\order{1/r},
\end{align}
where the second superscript index in parentheses denotes the power of $r$. Making use of the expansion of $\hmn{}{1}$, obtained by setting the acceleration to zero in the results for $\hmn{E}{1}$ found in Sec.~\ref{buffer_expansion1}, one finds
\begin{align}
\ddR{\alpha\beta}{2,-4}{\hmn{}{1}} &= 2m^2\left(7\nhat_{ab}+\tfrac{4}{3}\delta_{ab}\right)x^a_\alpha x^b_\beta -2m^2t_\alpha t_\beta,\label{ddR0n4}
\end{align}
and
\begin{align}
\ddR{tt}{2,-3}{\hmn{}{1}} &= 3m\H{ij}{1,0}\nhat^{ij},\label{ddR0n3_tt}\\
\ddR{ta}{2,-3}{\hmn{}{1}} &= 3m\C{i}{1,0}\nhat_{a}^i,\\
\ddR{ab}{2,-3}{\hmn{}{1}} &= 3m\big(\A{}{1,0}+\K{}{1,0}\big)\nhat_{ab}-6m\H{i\langle a}{1,0}\nhat_{b\rangle}^i+m\delta_{ab}\H{ij}{1,0}\nhat^{ij},\label{ddR0n3_ab}
\end{align}
and
\begin{align}
\ddR{tt}{2,-2}{\hmn{}{1}} &= -\tfrac{20}{3}m^2\etide_{ij}\nhat^{ij}+3m\H{ijk}{1,1}\nhat^{ijk}
+\tfrac{7}{5}m\A{i}{1,1}n^i+\tfrac{3}{5}m\K{i}{1,1}n^i\nonumber\\
&\quad-\tfrac{4}{5}m\partial_t\C{i}{1,0}n^i,\label{ddR0n2_tt}\\
\ddR{ta}{2,-2}{\hmn{}{1}}&= -m\partial_t\K{}{1,0}n_a+3m\C{ij}{1,1}\nhat_{a}{}^{ij}
+m\Big(\tfrac{6}{5}\C{ai}{1,1}-\partial_t\H{ai}{1,0}\Big)n^i\nonumber\\
 &\quad+2m\epsilon_a{}^{ij}\D{i}{1,1}n_j+\tfrac{4}{3}m^2\epsilon_{aik}\btide^k_j\nhat^{ij},\\
\ddR{ab}{2,-2}{\hmn{}{1}} &= \delta_{ab}m\left(\tfrac{16}{15}\partial_t\C{i}{1,0} -\tfrac{13}{15}\A{i}{1,1} -\tfrac{9}{5}\K{i}{1,1}\right)n^i\nonumber\\
&\quad+\delta_{ab}\left(-\tfrac{50}{9}m^2\etide_{ij}\nhat^{ij}+m\H{ijk}{1,1}\nhat^{ijk}\right) -\tfrac{14}{3}m^2\etide_{ij}\nhat_{ab}{}^{ij}\nonumber\\
&\quad+m\left(\tfrac{33}{10}\A{i}{1,1}+\tfrac{27}{10}\K{i}{1,1} -\tfrac{3}{5}\partial_t\C{i}{1,0}\right)\nhat_{ab}{}^i\nonumber\\
&\quad+m\left(\tfrac{28}{25}\A{\langle a}{1,1}-\tfrac{18}{25}\K{\langle a}{1,1}-\tfrac{46}{25}\partial_t\C{\langle a}{1,0}\right)\nhat^{}_{b\rangle}\nonumber\\
&\quad-\tfrac{8}{3}m^2\etide_{i\langle a}\nhat_{b\rangle}{}^i-6m\H{ij\langle a}{1,1}\nhat^{}_{b\rangle}{}^{ij}+3m\epsilon_{ij(a}\nhat_{b)}{}^{jk}\I{ik}{1,1} \nonumber\\
&\quad+\tfrac{2}{45}m^2\etide_{ab}-\tfrac{2}{5}m\H{abi}{1,1}n^i +\tfrac{8}{5}m\epsilon^i{}_{j(a}^{}\I{b)i}{1,1}n^j.\label{ddR0n2_ab}
\end{align}

I require an analogous expansion of $E\coeff{0}_{\alpha\beta}\left[\frac{1}{r^2}\hmn{}{2,-2} +\frac{1}{r}\hmn{}{2,-1}\right]$, where $E\coeff{0}_{\alpha\beta}[f]$ is defined for any $f$ by setting the acceleration to zero in $E_{\alpha\beta}[f]$. The coefficients of the $1/r^4$ and $1/r^3$ terms in this expansion can be found in Sec.~\ref{buffer_expansion2}; the coefficient of $1/r^2$ will be given here. For compactness, I define  this coefficient to be $\tilde E_{\alpha\beta}$. The $tt$-component of this quantity is given by  
\begin{align}
\tilde E_{tt} &= 2\partial^2_tM_in^i+\tfrac{8}{5}S^j\btide_{ij}n^i-\tfrac{2}{3}M^j\etide_{ij}n^i +\tfrac{82}{3}m^2\etide_{ij}\nhat^{ij} + 24S_{\langle i}\btide_{jk\rangle}\nhat^{ijk}\nonumber\\
&\quad-20M_{\langle i}\etide_{jk\rangle}\nhat^{ijk}.\label{E_tt}
\end{align}
The $ta$-component is given by
\begin{align}
\tilde E_{ta} &= \tfrac{44}{15}\epsilon_{aij}M^k\btide^j_kn^i -\tfrac{2}{15}\left(11S^i\etide^j_k+18M^i\btide^j\right)\epsilon_{ija}n^k +\tfrac{2}{15}\left(41S^j\etide^k_a -10M^j\btide^k_a\right)\epsilon_{ijk}n^i\nonumber\\
&\quad +4\epsilon_{aij}\left(S^j\etide_{kl} +2M_k\btide^j_l\right)\nhat^{ikl}+4\epsilon^{}_{ij\langle k}\etide_{l\rangle}^jS^i\nhat_a{}^{kl} +\tfrac{68}{3}m^2\epsilon_{aij}\btide^j_k\nhat^{ik}.
\end{align}
This can be decomposed into irreducible STF pieces via the identities
\begin{align}
\epsilon_{aij}S^i\etide^j_k & = S^i\etide^j_{(k}\epsilon_{a)ij}+\tfrac{1}{2}\epsilon_{akj}S^i\etide_i^j\\
\epsilon_{aj\langle i}\etide_{kl\rangle}S^j&=\mathop{\STF}_{ikl}\!\left[\epsilon^j{}_{al}S_{\langle i}\etide_{jk\rangle} -\tfrac{2}{3}\delta_{al}S^p\etide^j_{(i}\epsilon^{}_{k)jp}\right]\\
\epsilon_{aj\langle i}M_l\btide_{k\rangle}{}^j&=\mathop{\STF}_{ikl}\!\left[\epsilon^j{}_{al}M_{\langle i}\btide_{jk\rangle}\! +\!\tfrac{1}{3}\delta_{al}M^p\btide^j_{(i}\epsilon^{}_{k)jp}\right],
\end{align}
which follow from Eqs.~\eqref{decomposition_1} and \eqref{decomposition_2}, and which lead to
\begin{align}
\tilde E_{ta} &=\tfrac{2}{5}\epsilon_{aij}\Big(6M^k\btide^j_k-7S^k\etide^j_k\Big)n^i+\tfrac{4}{3}\left(2M^l\btide^k_{(i} -5S^l\etide^k_{(i}\right)\epsilon^{}_{j)kl}\nhat_a{}^{ij} \nonumber\\
&\quad+\left(4S^j\etide^k_{(a} -\tfrac{56}{15}M^j\btide^k_{(a}\right)\epsilon_{i)jk}n^i + 4\epsilon_{ai}{}^l\left(S_{\langle j}\etide_{kl\rangle}+2M_{\langle j}\btide_{kl\rangle}\right)\nhat^{ijk}\nonumber\\
&\quad+\tfrac{68}{3}m^2\epsilon_{aij}\btide^j_k\nhat^{ik}.\label{E_ta}
\end{align}
The $ab$-component is given by
\begin{align}
\tilde E_{ab} &= \tfrac{56}{3}m^2\etide_{ij}\nhat_{ab}{}^{ij} +\tfrac{52}{45}m^2\etide_{ab}-\delta_{ab}\left[\left(2\partial^2_tM_i+\tfrac{8}{5}S^j\btide_{ij} +\tfrac{10}{9}M^j\etide_{ij}\right)n^i+\tfrac{100}{9}m^2\etide_{ij}\nhat^{ij}\right] \nonumber\\
&\quad -\delta_{ab}\left(\tfrac{20}{3}M_{\langle i}\etide_{jk\rangle} -\tfrac{8}{3}S_{\langle i}\btide_{jk\rangle}\right)\nhat^{ijk}+\tfrac{8}{15}M_{\langle a}\etide_{b\rangle i}n^i+\tfrac{8}{15}M^i\etide_{i\langle a}n_{b\rangle}+\tfrac{56}{3}m^2\etide_{i\langle a}\nhat^{}_{b\rangle}{}^i\nonumber\\
&\quad+16M_i\etide_{j\langle a}\nhat_{b\rangle}{}^{ij}-\tfrac{32}{5}S_{\langle a}\btide_{b\rangle i}n^i+\tfrac{4}{15}\left(10S_i\btide_{ab}+27M_i\etide_{ab}\right)n^i\nonumber\\
&\quad+\tfrac{16}{3}S^i\btide_{i\langle a}n_{b\rangle}-8\epsilon_{ij\langle a}\epsilon_{b\rangle kl}S^j\btide^l_m\nhat^{ikm}+\tfrac{16}{15}\epsilon_{ij\langle a}\epsilon_{b\rangle kl}S^j\btide^{il}n^k.
\end{align}
Again, this can be decomposed, using the identities
\begin{align}
S_{\langle a}\btide_{b\rangle i} &=S_{\langle a}\btide_{bi\rangle} +\mathop{\STF}_{ab}\tfrac{1}{3}\epsilon_{ai}{}^j\epsilon_{kl(b} \btide_{j)}{}^lS^k +\tfrac{1}{10}\delta_{i\langle a}\btide_{b\rangle j}S^j,\\
S_i\btide_{ab} &=S_{\langle a}\btide_{bi\rangle} -\mathop{\STF}_{ab}\tfrac{2}{3}\epsilon_{ai}{}^j\epsilon_{kl(b} \btide_{j)}{}^lS^k +\tfrac{3}{5}\delta_{i\langle a}\btide_{b\rangle j}S^j,\\
\epsilon_{ij\langle a}\epsilon_{b\rangle kl}S^j\btide^{il} & = \mathop{\STF}_{ab}\epsilon_{akj}S^l\btide^i_{(j}\epsilon^{}_{b)il} -\tfrac{1}{2}\delta_{k\langle a}\btide_{b\rangle i}S^i,\\
\mathop{\STF}_{ikm}\epsilon_{ij\langle a}\epsilon_{b\rangle kl}S^j\btide^l_m & = \mathop{\STF}_{ikm}\mathop{\STF}_{ab}\Big(2\delta_{ai}S_{\langle b}\btide_{km\rangle}+\tfrac{1}{3}\delta_{ai}\epsilon^l{}_{bk}S^j \btide^p_{(l}\epsilon^{}_{m)jp}\nonumber\\
&\quad-\tfrac{3}{10}\delta_{ai}\delta_{bk}\btide_{mj}S^j\Big),
\end{align}
which lead to
\begin{align}
\tilde E_{ab} & = -2\delta_{ab}\left[\left(\partial^2_tM_i+\tfrac{4}{5}S^j\btide_{ij} +\tfrac{5}{9}M^j\etide_{ij}\right)n^i +\left(\tfrac{10}{3}M_{\langle i}\etide_{jk\rangle} -\tfrac{4}{3}S_{\langle i}\btide_{jk\rangle} \right)\nhat^{ijk}\right]\nonumber\\
 &\quad-\tfrac{100}{9}\delta_{ab}m^2\etide_{ij}\nhat^{ij}+\tfrac{1}{5}\left(8M^j\etide_{ij} +12S^j\btide_{ij}\right)\nhat_{ab}{}^i +\tfrac{56}{3}m^2\etide_{ij}\nhat_{ab}{}^{ij}\nonumber\\
&\quad +\tfrac{4}{75}\left(92M^j\etide_{j\langle a} +108S^j\btide_{j\langle a}\right)n_{b\rangle}^{} +\tfrac{56}{3}m^2\etide_{i\langle a}\nhat_{b\rangle}{}^i \nonumber\\
&\quad+16\mathop{\STF}_{aij}\left(M_i\etide_{j\langle a}-S_i\btide_{j\langle a}\right)\nhat^{}_{b\rangle}{}^{ij} -\tfrac{8}{3}\epsilon^{pq}{}_{\langle j}\left(2\etide_{k\rangle p}M_q+\btide_{k\rangle p}S_q\right)\epsilon^k{}_{i(a}\nhat_{b)}{}^{ij}  \nonumber\\
&\quad +\tfrac{16}{15}m^2\etide_{ab}+\tfrac{4}{15}\left(29M_{\langle a}\etide_{bi\rangle}-14S_{\langle a}\btide_{bi\rangle}\right)n^i \nonumber\\
&\quad-\tfrac{16}{45}\mathop{\STF}_{ab}\epsilon_{ai}{}^jn^i\epsilon^{pq}{}_{(b} \left(13\etide_{j)q}M_p+14\btide_{j)q}S_p\right).\label{E_ab}
\end{align}

